Improving Generalization by Incorporating Coverage in Natural Language Inference

The task of natural language inference (NLI) is to identify the relation between the given premise and hypothesis. While recent NLI models achieve very high performance on individual datasets, they fail to generalize across similar datasets. This indicates that they are solving NLI datasets instead of the task itself. In order to improve generalization, we propose to extend the input representations with an abstract view of the relation between the hypothesis and the premise, i.e., how well the individual words, or word n-grams, of the hypothesis are covered by the premise. Our experiments show that the use of this information considerably improves generalization across different NLI datasets without requiring any external knowledge or additional data. Finally, we show that using the coverage information is not only beneficial for improving the performance across different datasets of the same task. The resulting generalization improves the performance across datasets that belong to similar but not the same tasks.

==> Coverage%20for%20Robustness(2)/NLI.tex <==
\section{Natural Language Inference}
The task of natural language inference, or previously known as recognizing textual entailment, 

\paragraph{Baselines}
\begin{itemize}
    \item DecaNLP
    \item ??
\end{itemize}

\paragraph{Evaluation}

\begin{itemize}
    \item SNLI, MultiNLI
    \item \url{https://github.com/easonnie/analyze-compositionality-sensitivity-NLI}
    \item \url{https://abhilasharavichander.github.io/NLI\_StressTest/}
    \item Dataset of \cite{mccoy2018non}
    \item Cross-dataset evaluation?
\end{itemize}

\begin{table*}[htb]
\centering
\begin{tabular}{ l|l|llll }
 \hline
 \hline
 & \multicolumn{1}{c|}{in-domain} & \multicolumn{4}{c}{out-of-domain} \\ \hline
 & MultiNLI & SNLI & SNLI-lexical & stress-test & sick \\
 decaNLP (101000itr.) & 72.30 & 60.91 & 41.82 & 63.71 & 53.95 \\
 decaNLP (81000itr.) & &60.02 & 64.31 & 42.60 & 56.57  \\ 
 %+unigram-coverage & \\
 \quad + coverage & 73.84 & 65.38 & 78.69 & 63.74 & 54.55  \\
 %+cove & 74.78 & 63.53 & 67.71 & \\
 %+cove(50000) & 74.60 & \\
%  \hline 
%  \hline
%  ESIM & 77.45 & 66.91 & 67.54& 65.58 & 53.20\\
%  +coverage (glove?) & \\
 \hline
 \hline
 ESIM  & 79.81 & 69.85 & 62.69 & 63.28 & 53.01\\
 \quad + uni-coverage & 79.81 & 70.33 & 64.82 & 62.45 & 51.89\\
  \quad + coverage & & 70.05 & 67.47 & 69.32 & 52.65\\

 \hline
\end{tabular}
\caption{Performance of baseline NLI systems compared to their variation in which coverage values and indices are incorporated across various datasets. All models are trained on ``multinli'' training data. ``in-domain'' results show the performance on the multinli development set.}
\end{table*}

\begin{table*}[htb]
\centering
\begin{tabular}{ l|l|llll }
 \hline
 \hline
 & \multicolumn{1}{c|}{in-domain} & \multicolumn{4}{c}{out-of-domain} \\ \hline
 & SNLI & multiNLI & SNLI-lexical & stress-test & sick \\
 decaNLP  & 84.77 & 58.89 & 59.02 & 54.39 & 51.36\\
 \quad + coverage & 84.97 & 59.47 & 63.05 & 54.92 & 50.22 \\
 \hline \hline

 ESIM + ELMo & 88.92 & 64.56 & 66.39 & 52.61 & 56.51 \\
 \quad + uni-coverage & 88.72 & 63.89 & 69.38 & 53.2 & 56.91 \\
 %\quad + coverage & \textcolor{red}{89.04\%} & \textcolor{red}{63.6\%} & \textcolor{red}{67.18\%} & \textcolor{red}{51.22\%} & \textcolor{red}{55.83\%} \\
 \quad + coverage & 88.80 & 64.36 & 74.76& 57.34 & 56.84\\

 \hline
\end{tabular}
\caption{Performance of baseline NLI systems compared to their variation in which coverage values and indices are incorporated across various datasets. All models are trained on ``SNLI'' training data. ``in-domain'' results show the performance on the SNLI development set.}
\end{table*}

\paragraph{Analysis}
On which cases coverage feature help

==> Coverage%20for%20Robustness(2)/baselines.tex <==
\paragraph{Baseline Models.}
We incorporate coverage in two NLI models including:%\footnote{Both models are depicted in supplementary materials.}
\squishlist
\item \textbf{ESIM} \cite{P17-1152}, which is one of the top-performing systems on both SNLI and MultiNLI datasets.\footnote{E.g., its performance with ELMO embeddings and ensemble methods is 89.3 on SNLI.} We also use {ELMO} embeddings \cite{N18-1202} for this system.\footnote{ESIM and BIDAF models (with ELMO) are available at \url{https://github.com/allenai/allennlp}.}
%The structure of this network is shown in Figure~\ref{}.
%As we see, ESIM applies an average and maximum pooling layer on input encodings before the final softmax layer.

%ESIM first encodes both the premise and hypothesis using LSTM networks.
%They compute a soft alignment (attention) between the encoded words of premise and hypothesis.
%The attention weights are used for computing an attended representation for each sentence, e.g., a representation of the premise in which its relation with the hypothesis is also taken into account.
%The encoded and attended representations are fed into another network, and then a fix-size representation of each of the sentences will be computed by applying maximum and average pooling layers.
\item \textbf{MQAN }\cite{McCann2018decaNLP}, which is a sequence-to-sequence model with attention mechanisms and pointer networks \cite{vinyals2015pointer}. \newcite{McCann2018decaNLP} propose to model various NLP tasks as question answering so that we can apply a single model to various NLP tasks. 
%The architecture of MQAN is shown in Figure~\ref{}.
For the task of NLI, the question would be the hypothesis, and the context is the premise.
The main difference of this architecture compared to ESIM, or similar models, e.g., \newcite{D16-1244}, 
is that it uses the encoding of all the hypothesis words as the input to the decoder.
However, in the ESIM architecture, the encoding of individual words is not used for the final decision.
Instead, each sentence representation is summarized into a fixed vector using maximum and average pooling.
%\footnote{The architecture of these two models are included in supplementary materials.}
\squishend

==> Coverage%20for%20Robustness(2)/conc.tex <==
\section{Conclusions}
Despite the great progress in individual NLP datasets, current models do not generalize well across similar datasets, indicating that we are solving datasets instead of tasks.
Existing NLP methods mainly rely on the lexical form of the inputs, assuming that the required abstract knowledge is learned implicitly by the model.
In this paper, we propose a simple method that requires no additional data or external knowledge, to improve generalization.
We propose to extend the input encodings with a higher-level information regarding the relation of the input pairs, e.g., the hypothesis and the premise in NLI.
We show that the proposed solution considerably improves the performance (1) across datasets that represent the same task, and (2) across different datasets that represent similar tasks.
%For this purpose, we use coverage information, i.e., how well the hypothesis (query) aspects are covered by the premise (passage).
%providing the models with a higher level representation regarding the relation of input pairs in the existing datasets.
%We show the effectiveness of enriching inputs with coverage information in various NLI and QA models and datasets.


==> Coverage%20for%20Robustness(2)/generalization.tex <==
\section{Impact on Generalization}

\subsection{Baseline Systems}

\subsection{Evaluation Setting}

\subsection{Results}

\begin{table}[htb]
\centering
\resizebox{\columnwidth}{!}{%

\begin{tabular}{ l|ll|ll }
 \hline
 \hline
 & \multicolumn{2}{c|}{in-domain} &  \multicolumn{2}{c}{out-of-domain}  \\ 
 & \multicolumn{2}{c|}{SquAD}  & \multicolumn{1}{c}{QASRL} & \multicolumn{1}{c}{ZRE} \\ 
 \hline
 & EM & F1 & F1 & corpus-F1  \\
 base & 31.76& 75.37 & 50.10 & 27.16\\
 +coverage & 32.67 & 76.83 & 50.89 & 32.79 \\ 
+answer generation & \\
 %\quad answer generation+c & 32.50 & 76.05 & \\
\hline
\end{tabular}
}
\caption{Impact of coverage vs.\ full answer generation on improving generalization of decaNLP.}
\end{table}

\begin{table}[htb]
\centering
\resizebox{\columnwidth}{!}{%

\begin{tabular}{ l|ll|llll }
 \hline
 & \multicolumn{2}{c|}{in-domain} &  \multicolumn{4}{c}{out-of-domain}  \\ 
 & \multicolumn{2}{c|}{SquAD}  & \multicolumn{2}{c}{QASRL} & \multicolumn{2}{c}{ZRE} \\ 
 \hline
  & EM & F1 & EM & F1 & EM & F1  \\
 \hline
 base & 70.43 & 79.76 & & 50.01 & & \textcolor{red}{36.18} \\
 +coverage & 71.07 & 80.15 & & \textcolor{red}{52.24} & & \textcolor{red}{35.25}\\

 
\hline
\end{tabular}
}
\caption{Effect of incorporating coverage on the BiDAF QA model.}

\end{table}

==> Coverage%20for%20Robustness(2)/how.tex <==
\section{How to Better Understand the Question?}
As mentioned, artifacts in existing datasets drives QA models to learn datasets instead of the task itself.


We examined two different approach in order to improve the understanding of the model from the given question: (1) incorporating a more abstract knowledge about the question into the model, i.e., coverage of the question aspects by the answer, and (2) regenerating a full sentence for answering the question instead of only selecting the answer span.





==> Coverage%20for%20Robustness(2)/intro.tex <==
\section{Introduction}
%In order to facilitate the advances in various NLP applications, creating large-scale datasets using crowdsourcing has became more popular.
The task of Natural language inference (NLI) \cite{W03-0906,dagan2006pascal,D15-1075} is to specify whether the given hypothesis entails, contradicts, or is neutral regarding the premise.
While existing NLI models have high performances on individual datasets,\footnote{E.g. 91\% accuracy on the SNLI dataset \cite{liu2019multi}.} they fail to generalize across different datasets of the same task.
%As a result, the progress on such datasets, may be the result of overfitting to the dataset, and its artifacts, and not the general progress on solving the task itself.
This indicates that existing models are overfitting to specific properties of each dataset instead of learning the higher-level inference knowledge that is required to solve the task. 
%In particular, it is shown that the largest available NLI datasets, which are the basis for evaluating progress in this field, contain artifacts that are easily exploitable by neural models \cite{N18-2017}. %,S18-2023 therefore, do not well present the natural distributions of the task.

Existing solutions to improve the performance of NLI models across datasets include (1) using external knowledge \cite{joshi2018pair2vec,P18-1224}, and (2) fine-tuning on the target datasets, e.g., \cite{bansal:AAAI:2019,liu2019inoculation}.
The above approaches include the use of additional data or knowledge sources. Besides, fine-tuning on one target dataset may decrease the performance on the other datasets \cite{bansal:AAAI:2019}.

%In order to show that current models capture dataset- or word-level information, instead of high-level inference knowledge, several adversarial variations of NLI datasets are proposed, each of them reveals a specific weakness of NLI models or datasets, e.g., \cite{mccoy2019right,C18-1198,P18-2103}.
%The common approach to address the identified weaknesses is adversarial data augmentation, i.e., to integrate adversarially augmented data into the training data so that the model's performance improves on augmented weaknesses.
%The limitation of adversarial augmentation is its narrow scope. Training on one type of adversarially augmented data does not generalize to, and in fact decreases the performance on, other types of adversaries \cite{bansal:AAAI:2019}.
%Another approach to improve generalization is to incorporate background knowledge \cite{joshi2018pair2vec,P18-1224}, which requires using external resources.
In this paper, we propose a simple approach to improve generalization by using the information that is \emph{already present} in the dataset.
Existing NLI methods overly rely on the lexical form of the inputs, assuming that the model itself learns the required abstractions.
Instead, we propose to extend the existing input representations with a more abstract view of the relation between the hypothesis and premise, i.e., how well each word, or word n-gram, of the hypothesis is covered by the premise.
Our experiments show that using this information considerably and consistently improves generalization across various NLI datasets, i.e., from one to 30 points improvements.% in out-of-domain evaluations.

Finally, we show that beside improving the performance across different datasets of the same task, our proposed approach also improves the performance across datasets of similar tasks, i.e., reading comprehension on the SQuAD dataset and QA-SRL \cite{he-etal-2015-question}.
%Our results show that by using the coverage information, the performance of a model that is trained for the task of reading comprehension improves on the dataset of a similar but different task, i.e., QA-SRL. % for   but also across datasets of similar tasks we show that incorporating this coverage information in question answering models, by including how well each aspect of the question is covered by the candidate passage, also improves generalization of the examined QA systems across similar datasets.
%Overall, the \textbf{benefit} of the proposed solution is that while it does \emph{not require any external knowledge or additional annotated data}, it considerably \emph{improves generalization} and therefore, the cross-dataset performance.  
%Existing NLI models already rely on computing the similarity of the hypothesis words to those of the premise.
%However, we show that if we explicitly extend the representation of each word in the hypothesis by (1) its maximum similarity value to the premise words, and (2) the position of the most similar word of the premise, generalization improves considerably and consistently across various datasets, i.e., from one to 30 points improvements in out-of-domain evaluations.    
%Existing NLI approaches overly rely on the lexical forms of the inputs, assuming that the model itself learns the required abstractions.
%Instead, we extend the existing input encodings with a more abstract representation about the relation between the hypothesis and premise, i.e., how well each word of the hypothesis is covered by the premise.
%Our experiments show that using coverage information considerably and consistently improves the generalization of the examined NLI models across various datasets, i.e., from one to 30 points improvements in out-of-domain evaluations.
%The results indicate that incorporating coverage helps the model to learn dataset-independent knowledge that is also transferable to other datasets.

%We then show that using coverage information also benefits.
%Finally, we show that incorporating the maximum similarity values for question answering, i.e., maximum similarity of each word of the question to those of the passage, also improves the generalization across similar datasets.
%, by including how well each aspect of the question is covered by the candidate passage, also improves generalization of the examined QA systems across similar datasets.
%The code of all of our experiments with coverage information will be released upon the publication.

%The code of all of our experiments with the coverage information will be released upon the publication.

%As mentioned above, as a result of dataset artifacts, models tend to learn specific properties of the datasets instead of the knowledge which is required for solving the general task.

%Our analyses show that 



%While there has been a great progress in these datasets, e.g., 91\% accuracy on SNLI \cite{D15-1075}, 

%for the task of natural language inference \cite{liu2019multi}, and human-performance level on the SQuAD dataset \cite{D16-1264} for question answering \cite{devlin2018bert}.

%However, some datasets that are used to measure the progress contain artifacts \cite{N18-2017,D18-1546}, and therefore, do not well present the natural distributions of their corresponding tasks.
%As a result, the progress on a particular dataset, may be the result of overfitting to the dataset, and its artifacts, and not the general progress on solving the task that the dataset presents.


%One way to help the model to generalize better and to learn higher-level knowledge, 
%is simply to incorporate more abstract information from the inputs.


%Each word of the hypothesis, in common NLI models, is represented based on its own embedding 
%as well its alignments with the premise words. 


%we propose to also incorporate this information for the task of NLI to provide the model with a more abstract view of the hypothesis relation to the premise.

%\newcite{rueckle:AAAI:2019} compute how well each aspect, i.e., bigram, of the query is covered by the candidate answer and they select the candidate answer that covers most aspects of the query.
%They show that this models outperforms various semantic similarity methods, in which a semantic representation is computed for the query and each candidate answer and the answer whose representation is the most similar to that of the query will be selected as the correct answer.


%In this paper we first propose to incorporate coverage information in NLI models, i.e., how well each aspect of the hypothesis is covered by the premise, and where are the premise aspects that best cover those of hypothesis.
%We show that while the incorporation of coverage information does not increase the complexity of the model,\footnote{??} it significantly improves the generalization of the model.

%The generalization is measured by training the model on one dataset, and evaluating it on other datasets from the same task, so that we can evaluate whether the model learns dataset-independent knowledge that is also transferable to other datasets.
%\todo{numbers}






==> Coverage%20for%20Robustness(2)/method.tex <==
\definecolor{one}{rgb}{1.0, 0.64,0.45}
\definecolor{two}{rgb}{0.96, 0.45,0.38}
\definecolor{three}{rgb}{0.86, 0.27,0.32}
\definecolor{four}{rgb}{0.55, 0.0,0.0}


\begin{table*}[htb]
    \centering
    \footnotesize
    %\resizebox{\textwidth}{!}{%

    \begin{tabular}{|l|l| l|}
 \hline
                   P & [\textcolor{one}{{The man}}] [\textcolor{two}{\textbf{spoke}}] to [\textcolor{three}{\textbf{the lady}}] with the [\textcolor{four}{\textbf{red dress}}].  & \textbf{label}\\ \hline

         H$_1$&  [\textcolor{one}{{The man}}] [\textcolor{two}{\textbf{talked}}] to [\textcolor{three}{\textbf{the woman}}] in [\textcolor{four}{\textbf{red cloth}}]. & entail \\
         H$_2$&  [\textcolor{one}{{The man}}] did \textbf{not} [\textcolor{two}{\textbf{talk}}] to [\textcolor{three}{\textbf{the woman}}] in [\textcolor{four}{\textbf{red dress}}]. & contradict \\
         H$_3$& [\textcolor{three}{\textbf{The woman}}] [\textcolor{two}{\textbf{lectured}}] [\textcolor{one}{{the man}}]. & neutral \\ \hline
    \end{tabular}
    %}
    \caption{A sample premise and three hypotheses. Matching words, e.g., ``spoke'' and ``talked'', and bigrams, e.g., ``red dress'' and ``red cloth'', are specified by the same color.}
    \label{tab:coverage_exm}
\end{table*}



\section{Enhancing Word Representations with Coverage Information}
Assume $P$ and $H$ are the premise and the hypothesis, respectively, and $\Phi(P)\in \mathbb{R}^{|P|\times d}$ and $\Phi(H) \in \mathbb{R}^{|H|\times d}$ are their corresponding learned representations, e.g., $\Phi_i(H)$ is the representation of the $i$th word of the hypothesis.
The similarity matrix is computed as $S=\Phi(H)\Phi(P)^T$, where $S_{ij}$ shows the similarity of the $i$th word of $H$ to the $j$th word of $P$.\footnote{Such a similarity matrix is already used in various NLI models, e.g., our baseline models, for computing word alignments and attention weights.}

The \textbf{coverage values} are computed as $c_i = max_j(S_{ij})$.
$c_i$ is the maximum similarity of the $i$th word of $H$ to the premise words indicating how well the $i$th word is covered by $P$.
%indicates how well the $i$th aspect of $H$ is covered by the premise.

Moreover, we can compute the coverage values for n-grams, i.e., $\Phi_i^\prime(H)$ is the learned representation of the word n-gram of the hypothesis that starts with the word $i$ and $c^\prime_i$ is the maximum similarity of this n-gram to the n-grams of the premise.
In this work, we use bigrams and we use a CNN with the window size two for computing $\Phi^\prime$.
The use of coverage values is motivated by the success of the relevance matching model of \newcite{rueckle:AAAI:2019} for the task of answer ranking in community question answering.
%Given a query and a set of candidate answers, the task is to rank candidate answers based on their relevance to the query.
\newcite{rueckle:AAAI:2019} rank candidate answers based on on their coverage of the question bigrams.
%They consider aspects as learned representations of bigrams, which is computed using a Convolutional Neural Network with the window size two.
%In this work, we evaluate three aspect variations including: (1) unigrams,  (2) bigrams\footnote{Which are computed similar to \newcite{rueckle:AAAI:2019}.},  and (3) both\footnote{One similarity matrix for unigrams and one for bigrams.}.
Beside coverage values, we can also benefit from \textbf{coverage positions}, i.e., \mbox{$q_{i}=\argmax_j (S_{ij})$}, 
which specifies the position of the premise word (n-gram) that has the highest similarity with the $i$th word (n-gram) of $H$. 


Table~\ref{tab:coverage_exm} shows a premise and three different hypotheses with their corresponding labels.
The best matching words or bigrams of the hypotheses and the premise are specified with the same colors.

For instance, in H$_2$, ``talked'' is best covered by ``spoke'' in $P$. However, the word ``not'' and the bigram ``not talked'' are not well covered by $P$.
The use of coverage values can highlight these non-covered words in H$_2$.
On the other hand, all words and bigrams of $H_3$ have high similarity (coverage) with those of the premise. However, they are not covered in the right order. The incorporation of coverage positions can help the detection of such cases, e.g., in H$_3$, the first bigram is best covered at position five of P while the last bigram is covered at position zero.

%For instance, the coverage indices for the three specified bigrams in $H_3$ are 6, 3, and 2, which inform the model that these aspects are not covered in the right order.
%using coverage index can inform the model that while ``the woman'' appears in the beginning of $H_3$, it is covered by an aspect that appears towards the end of $P$, i.e., sixth bigram.

%Following \newcite{rueckle:AAAI:2019}, we consider unigram and bigrams as aspects.


\paragraph{How to Incorporate Them?}
Assume $C$ and $C^\prime$ are the coverage vectors based on the words and bigrams of the hypothesis, respectively, e.g., $c_i \in C$ is the coverage value for the $i$th word.
Similarly, let $Q$ and $Q^\prime$ be the corresponding position vectors for $C$ and $C^\prime$.

The default setting in all of our experiments is to use  only $C$, and we consider the inclusion of the $C^\prime$, $Q$, and $Q^\prime$ vectors as hyper-parameters of the model.
The other hyper-parameter is the learned representation for computing the coverage vectors, i.e., $\Phi$, that can be the input embeddings or the output of any of the intermediate layers of the network that encode the input sentences.
%For a model that have several layers for encoding each word, the resulting representation from each of those layers can be used as $\Phi$.
We determine these two parameters based on the performance on the (in-domain) development set.

%There are several layers to encode the premise and th
%hypothesis, each of them can be used as word encodings.
%the rest of the three vectors by performing hyper-parameter optimization on the development set of the training data.
%Assume that we want to incorporate all the above four coverage vectors.
We then incorporate the coverage vectors\footnote{I.e., $C$ and those of $C^\prime$, $Q$, and $Q^\prime$ that are recognized beneficial based on the results on the development set.} by concatenating them with the learned representation of the hypothesis.
For instance, if we want to incorporate all the above vectors, the learned representation that is enhanced with the coverage information will be constructed as \mbox{$\Phi_{cov}=[\Phi(H);C;C^\prime;Q;Q^\prime] \in \mathbb{R}^{|H|\times (d+4)}$}.

The use of coverage vectors requires no change in the model architecture and the only difference is the dimensionality of the word representations from $d$ to $d+k$, where $1<k<4$, in a single layer of the network, i.e., the selected layer in which the coverage vectors are incorporated.
If the model uses the same network for encoding both $P$ and $H$, we concatenate zero values to the representation of $P$ to keep the dimensions the same for both.


%In all experiments, the coverage values (and coverage indices) are concatenated with the encoding of the hypothesis.
%and whether to use coverage indices, is made based on the performance on the development set.  
%In our preliminary experiments on incorporating coverage, we find a direct correlation between the improvements on the development set and the resulting improvements in generalization.
%For instance, ESIM summarizes the sequence of the hypothesis word encodings by using maximum and average pooling. Therefore, incorporating position information in such a model is not beneficial because it cannot be .


%The computed similarity matrix is commonly used for computing attentions and attended vectors for both inputs, e.g., question-to-passage or passage-to-question attentions \cite{bidaf,McCann2018decaNLP}.




==> Coverage%20for%20Robustness(2)/nli.tex <==
\section{Natural Language Inference}
\label{sect:nli}
\paragraph{Datasets.} The examined datasets are:
\squishlist
\item \textbf{SNLI} \cite{D15-1075} is large crowdsourced dataset in which premises are taken from image captions.
\item \textbf{MultiNLI} \cite{N18-1101} covers ten different genres but is otherwise similar to SNLI. 
Only five genres are included in the training data. The \textit{Matched} evaluation set contains the same genres as the training data while \textit{Mismatched} set includes different genres from those of training. 
\item \textbf{SICK} \cite{sick} is also a crowdsourced dataset using sentences that describe pictures or videos. It is smaller than the first two datasets. 
%\item RTE-3 test set \cite{dagan2006pascal}: this dataset is of higher quality and hand-labeled.
%It is created so that it simulates the logical and statistical modeling of natural language reasoning.
%The reason that this dataset is not used for training recent NLI models, is its small size.
\item \textbf{\newcite{P18-2103}} is an adversarially constructed dataset, in which premises are taken from SNLI and the hypotheses differ from the premise only by one word.
Compared to SNLI, it is an easier dataset for humans. However, the performance of NLI models considerably decreases on this dataset.
\squishend
\textbf{Dataset Artifacts.} The progress in NLI is mainly determined by SNLI and MultiNLI.
These datasets are created by presenting the annotators with a premise and asking them to create three hypotheses with entailment, contradiction, and neutral labels.
This dataset creation method results in various artifacts, e.g., identifying the label by only using the hypothesis \cite{S18-2023,N18-2017}.
Similarly, the analysis of \newcite{C18-1198} suggests that models that rely on lexical overlap of premise and hypothesis and other shallow lexical cues can perform well on such datasets without performing higher-level reasoning.
Models that have high performance due to learning dataset artifacts, can be easily compromised by adversarial or more challenging examples \cite{bansal:AAAI:2019,mccoy2019right,mccoy2018non,P18-2103,C18-1198}. 
Improving the generalization of NLI models across different datasets, which presumably contain different kinds of annotation biases, is a promising direction to abstract away from dataset-specific artifacts.

\input{baselines.tex}
\paragraph{Evaluation Metric.} Similar to previous work, we use the classification accuracy for evaluation.



==> Coverage%20for%20Robustness(2)/nli_res.tex <==
\begin{table*}[htb]
\centering
%\resizebox{\columnwidth}{!}{%

\begin{tabular}{ l|l|lll}

 \hline
 & \multicolumn{1}{c|}{in-domain} & \multicolumn{3}{c}{out-of-domain} \\ \hline
 & MultiNLI & SNLI & Glockner & SICK \\ \hline
 MQAN & 72.30 & 60.91 & 41.82 & 53.95 \\
% decaNLP (81000itr.) & &60.02 & 64.31 & 42.60 & 56.57  \\ 
 %+unigram-coverage & \\
 \quad + coverage & \textbf{73.84} & \textbf{65.38} & \textbf{78.69} & \textbf{54.55}  \\
 %both coverage & 73.23 & 64.57 & 58.37 & 63.53 & 51.42 \\
 %+cove & 74.78 & 63.53 & 67.71 & \\
 %+cove(50000) & 74.60 & \\
%  \hline 
%  \hline
%  ESIM & 77.45 & 66.91 & 67.54& 65.58 & 53.20\\
%  +coverage (glove?) & \\
 \hline

 %ESIM (?) & 79.81 & 69.85 & 62.69 & 53.01\\
 ESIM (ELMO) & 80.04 & 68.70 & 60.21 & 51.37\\
   \quad + coverage & \textbf{80.38} & \textbf{70.05} & \textbf{67.47} & \textbf{52.65}\\

 \hline
\end{tabular}
%}
\caption{Impact of using coverage for improving generalization across different datasets of the same task (NLI). All models are trained on MultiNLI.}
\label{nli_generalization_mnli}
\end{table*}


\section{Improving the Cross-Dataset Performance for the Same Task}
%In this section, we evaluate the use of coverage information on MQAN and ESIM models.
We train both NLI models on the MultiNLI training data.
As the development set, we use the concatenation of matched and mismatched splits of the MultiNLI development set.
%We then select our hyper-parameters, the inclusion of $C^\prime$, $P$, and $P^\prime$ as well as the layer of the network to incorporate the coverage vectors, on this development set. 
Based on the results on this development set, the use of $C^\prime$ is useful for both models.
However, incorporating $Q$ and $Q^\prime$ only benefits MQAN.
The reason is that ESIM summarizes the sequence of hypothesis words by using maximum and average pooling and these operations cannot handle position and ordering information.
MQAN has several decoding layers on top of the hypothesis representation, and therefore, it can make sense of the coverage positions.




Table~\ref{nli_generalization_mnli} shows the performance for both systems for in-domain (the MultiNLI development set) as well as out-of-domain evaluations on SNLI, Glockner, and SICK datasets.
%\footnote{We train each model multiple times.  For ``+coverage'' experiments, we observe a very low variance between different runs. For baselines, we report the evaluation of the model with the best development results.}

\begin{table*}[!htb]
\centering
%\resizebox{\columnwidth}{!}{%

\begin{tabular}{ l|rr|rr }
 & \multicolumn{2}{c|}{in-domain} &  \multicolumn{2}{c}{out-of-domain}  \\ 
 & \multicolumn{2}{c|}{SQuAD}  & \multicolumn{2}{c}{QA-SRL}  \\ 
 \hline
 & EM & F1 & EM & F1  \\ \hline
 MQAN & 31.76& 75.37 & \textbf{10.99} & 50.10 \\
 \quad +coverage & \textbf{32.67} & \textbf{76.83} & 10.63 & \textbf{50.89}  \\ \hline
 BIDAF (ELMO)& 70.43 & 79.76 & 28.35 & 49.98 \\
 \quad +coverage & \textbf{71.07} & \textbf{80.15} & \textbf{30.58} & \textbf{52.43}  \\
\hline
\end{tabular}
%}
\caption{Impact of using coverage for improving generalization across the datasets of similar tasks. Both models are trained on the SQuAD training data.}
\label{tab:qa_results}
\end{table*}

The results show that coverage information considerably improves the generalization of both examined models across various NLI datasets.
The resulting cross-dataset improvements on the SNLI and Glockner datasets are larger than those on the SICK dataset.
The reason is that the dataset creation process and therefore, the task formulation is similar in SNLI and MultiNLI, but they are different from SICK.
In particular, in the neutral pairs in SNLI and MultiNLI, the hypothesis is mostly irrelevant to the premise, e.g., ``He watched the river flow'' and ``The river levels were rising''.
However, in the SICK dataset, neutral pairs also have high lexical similarity, e.g., ``A woman is taking eggs out of a bowl'', and ``A woman is cracking eggs into a bowl''. 
As a result, a model that is trained on SNLI or MultiNLI does not learn to properly recognize the neutral pairs in the SICK dataset. 






==> Coverage%20for%20Robustness(2)/qa.tex <==


\section{Improving the Cross-Dataset Performance for Similar Tasks}
In this section, we examine whether we can benefit from the coverage information (1) in a task other than NLI, and (2) for improving performance across datasets that belong to similar but different tasks. 
%of question answering by incorporating how well each aspect of the question is covered by the given passage.
To do so, we select two related question answering tasks including reading comprehension and Question-Answer driven Semantic Role Labeling (QA-SRL) \cite{he-etal-2015-question}.
We train the baseline question answering models on a reading comprehension dataset and evaluate their performance on QA-SRL.

\paragraph{Datasets.} For training, we use the SQuAD dataset \cite{D16-1264}, in which a question and a passage are given and the task is to extract the answer from the passage.
%The SQuAD dataset is also created by crowdsourcing and contains known artifacts \cite{D18-1546}.

%In order to evaluate how well the model captures task-level, instead of dataset-level, question answering skills, we use the question-answer driven semantic role labeling (QA-SRL) dataset \cite{D15-1076} for evaluation.
%, and zero-shot relation extraction (ZRE) \cite{K17-1034}.
In QA-SRL, predicate-argument structures\footnote{I.e., ``who'' did ``what'' to ``whome''.} are present using natural question-answer pairs. For instance, in the sentence ``John published a comic book'', the predicate-argument structures for the verb ``published'' can be determined by answering the questions ``who published something?'' and ``what was published?''.
In this dataset, the wh-questions and  a sentence
%, from which such question-answer pairs are extracted,
are given and the task is to find the answer span from the sentence.

We hypothesize that if a model learns more abstract knowledge about answering questions from the SQuAD dataset, it can also perform better in answering the questions of QA-SRL.\footnote{This setting is also used for evaluating general linguistic intelligence by \newcite{yogatama2019learning}.}

%\newcite{K17-1034} model relation extraction as a reading comprehension task in which each relation slot is associated with one or more questions.
%For instance, the relation $spouse(John,y)$ can be defined by natural questions like ``who did John married?'' or ``who is John's spouse?''.
%The test data in ZRE contains new relation types that have no labeled training examples.

%While there are differences in the format of question in SQuAD, QA-SRL, and ZRE,
%if a model learns more abstract knowledge about answering questions from the given passage, it would perform better in of all these datasets.\footnote{This setting is also used for evaluating general linguistic intelligence by \newcite{yogatama2019learning}} 
%We use the standard evaluation metrics for each of the above tasks, i.e., exact match and F$_1$ in reading comprehension and QA-SRL, and corpus-F$_1$ in ZRE.  

\paragraph{Baselines.} We use BIDAF \cite{bidaf} with ELMO embeddings as well as MQAN as baselines.
Coverage vectors are computed based on the maximum similarity of the question words to those of the given context, i.e., a passage in SQuAD and a sentence in QA-SRL.
Based on the results on the SQuAD development set, incorporating $C^\prime$ coverage vector is useful for MQAN and BIDAF only benefits from using $C$.

%and incorporating only unigram coverage values in BIDAF are the best settings for QA experiments.
\paragraph{Results.}


Table~\ref{tab:qa_results} shows the impact of coverage for improving generalization across these two datasets that belong to the two similar tasks of reading comprehension and QA-SRL.
The models are evaluated using Exact Match (EM) and F$_1$ measures, which are the common metrics in QA.
The results are reported on the SQuAD development set and the QA-SRL test set. 
All models are trained on the SQuAD training data.
As the results show, incorporating coverage improves the model's performance in the in-domain evaluation as well as the out-of-domain evaluation in QA-SRL.
This indicates that more generalizable systems also improve the performance across related tasks.





  


==> Coverage%20for%20Robustness(2)/rel.tex <==
\section{Related Work}

==> Coverage%20for%20Robustness(2)/tasks.tex <==
\section{Tasks}
In this paper, we examined different tasks and datasets.
The examined tasks can be classified into two groups including: question answering and natural language inference.

For question answering, we consider the following tasks: (1) reading comprehension, (2) question-answer driven semantic role labeling (QA-SRL) \cite{D15-1076}, and (3) zero-shot relation extraction (ZRE) \cite{K17-1034}.

For the task of natural language inference, we examine various datasets including:

\paragraph{Reading Comprehension.} In this task a question and a related passage is given and the task is to extract the answer span from the passage.
For the task of reading comprehension, we use the the SQuAD dataset \cite{D16-1264}.
The performance of reading comprehension models is measured by the exact match, i.e., , and F$_1$, i.e., , measures.
%The SQuAD and NewsQA datasets are both created using crowdsourcing.
%SQuAD is created based on Wikipedia articles while NewsQA is created based on CNN news articles.

\paragraph{Question-answer driven semantic role labeling.} 
Semantic Role Labeling (SRL) is the task of finding the semantic arguments of a predicate (e.g.,\ verb) as well as their corresponding roles, e.g., agent, patient, instrument, etc.  
\newcite{D15-1076} propose the task of question-answer driven SRL, in which predicate-argument structures are presented using natural question-answer pairs. For instance, in the sentence ``Alan Turing published Intelligent machinery, a heretical theory'', ``published'' is a predicate with two different arguments, i.e., ``Alan Turing'' and ``Intelligent machinery, a heretical theory''. These predicate-argument structures can be presented by the following two question-answer pairs: (1) ``who published something?''-``Alan Turing'', and (2)``what was published?''-```Intelligent machinery, a heretical theory''.
In QA-SRL, a sentence, from which such question-answer pairs are extracted, and the wh-question question are given and the task is to find the answer span from the sentence.

\paragraph{Zero-shot relation extraction.}
\newcite{K17-1034} propose to model the task of relation extraction as a reading comprehension task in which each relation slot is associated with one or more questions.
For instance, the relation $spouse(x,y)$ can be defined by natural questions like ``who did $x$ married?'' or ``who is $x$'s spouse?''.
\newcite{K17-1034} provide a zero-shot relation extraction dataset with the aforementioned setting, in which the test data contains new relation types that have no labeled training examples.

\paragraph{Natural language inference.} 
Given two sentences, i.e., premise and hypothesis,
the task of natural language inference (NLI) is to specify whether the hypothesis entails, contradicts, or is neutral regarding the given premise.
We use different datasets including RTE-3 \cite{W07-1401}, Stanford NLI corpus (SNLI) \cite{D15-1075}, Multi-Genre NLI (MultiNLI) \cite{N18-1101}, Sentences Involving Compositional Knowldedge (SICK) \cite{sick}, as well as the test set that is created by \newcite{P18-2103}, which we would refer to as SNLI-adv.
The premises of the \newcite{P18-2103} dataset are taken from the SNLI dataset and the hypotheses only differ from the premise by one word.
While this dataset is simpler than SNLI, performance of existing NLI models drop significantly on this dataset.

%\squishlist
%\item Stanford NLI corpus (SNLI) \cite{D15-1075}: this dataset is a large crowdsourced dataset annotated with textual entailment information. The creation of this dataset is based on image captions, i.e., annotators were given a caption of an image and were asked to write an alternative caption that entails, contradicts , or is neutral regarding the original caption.
%\item Multi-Genre NLI (MultiNLI) \cite{N18-1101}: this corpus is also a crowd-sourced dataset, which is modeled on the SNLI dataset. The difference is that it covers a range of genres of spoken and written text.
%\item Sentences Involving Compositional Knowldedge (SICK) \cite{sick}: 
%\squishend




==> NLI.tex <==
\section{Natural Language Inference}
The task of natural language inference, or previously known as recognizing textual entailment, 

\paragraph{Baselines}
\begin{itemize}
    \item DecaNLP
    \item ??
\end{itemize}

\paragraph{Evaluation}

\begin{itemize}
    \item SNLI, MultiNLI
    \item \url{https://github.com/easonnie/analyze-compositionality-sensitivity-NLI}
    \item \url{https://abhilasharavichander.github.io/NLI\_StressTest/}
    \item Dataset of \cite{mccoy2018non}
    \item Cross-dataset evaluation?
\end{itemize}

\begin{table*}[htb]
\centering
\begin{tabular}{ l|l|llll }
 \hline
 \hline
 & \multicolumn{1}{c|}{in-domain} & \multicolumn{4}{c}{out-of-domain} \\ \hline
 & MultiNLI & SNLI & SNLI-lexical & stress-test & sick \\
 decaNLP (101000itr.) & 72.30 & 60.91 & 41.82 & 63.71 & 53.95 \\
 decaNLP (81000itr.) & &60.02 & 64.31 & 42.60 & 56.57  \\ 
 %+unigram-coverage & \\
 \quad + coverage & 73.84 & 65.38 & 78.69 & 63.74 & 54.55  \\
 %+cove & 74.78 & 63.53 & 67.71 & \\
 %+cove(50000) & 74.60 & \\
%  \hline 
%  \hline
%  ESIM & 77.45 & 66.91 & 67.54& 65.58 & 53.20\\
%  +coverage (glove?) & \\
 \hline
 \hline
 ESIM  & 79.81 & 69.85 & 62.69 & 63.28 & 53.01\\
 \quad + uni-coverage & 79.81 & 70.33 & 64.82 & 62.45 & 51.89\\
  \quad + coverage & & 70.05 & 67.47 & 69.32 & 52.65\\

 \hline
\end{tabular}
\caption{Performance of baseline NLI systems compared to their variation in which coverage values and indices are incorporated across various datasets. All models are trained on ``multinli'' training data. ``in-domain'' results show the performance on the multinli development set.}
\end{table*}

\begin{table*}[htb]
\centering
\begin{tabular}{ l|l|llll }
 \hline
 \hline
 & \multicolumn{1}{c|}{in-domain} & \multicolumn{4}{c}{out-of-domain} \\ \hline
 & SNLI & multiNLI & SNLI-lexical & stress-test & sick \\
 decaNLP  & 84.77 & 58.89 & 59.02 & 54.39 & 51.36\\
 \quad + coverage & 84.97 & 59.47 & 63.05 & 54.92 & 50.22 \\
 \hline \hline

 ESIM + ELMo & 88.92 & 64.56 & 66.39 & 52.61 & 56.51 \\
 \quad + uni-coverage & 88.72 & 63.89 & 69.38 & 53.2 & 56.91 \\
 %\quad + coverage & \textcolor{red}{89.04\%} & \textcolor{red}{63.6\%} & \textcolor{red}{67.18\%} & \textcolor{red}{51.22\%} & \textcolor{red}{55.83\%} \\
 \quad + coverage & 88.80 & 64.36 & 74.76& 57.34 & 56.84\\

 \hline
\end{tabular}
\caption{Performance of baseline NLI systems compared to their variation in which coverage values and indices are incorporated across various datasets. All models are trained on ``SNLI'' training data. ``in-domain'' results show the performance on the SNLI development set.}
\end{table*}

\paragraph{Analysis}
On which cases coverage feature help

==> generalization.tex <==
\section{Impact on Generalization}

\subsection{Baseline Systems}

\subsection{Evaluation Setting}

\subsection{Results}

\begin{table}[htb]
\centering
\resizebox{\columnwidth}{!}{%

\begin{tabular}{ l|ll|ll }
 \hline
 \hline
 & \multicolumn{2}{c|}{in-domain} &  \multicolumn{2}{c}{out-of-domain}  \\ 
 & \multicolumn{2}{c|}{SquAD}  & \multicolumn{1}{c}{QASRL} & \multicolumn{1}{c}{ZRE} \\ 
 \hline
 & EM & F1 & F1 & corpus-F1  \\
 base & 31.76& 75.37 & 50.10 & 27.16\\
 +coverage & 32.67 & 76.83 & 50.89 & 32.79 \\ 
+answer generation & \\
 %\quad answer generation+c & 32.50 & 76.05 & \\
\hline
\end{tabular}
}
\caption{Impact of coverage vs.\ full answer generation on improving generalization of decaNLP.}
\end{table}

\begin{table}[htb]
\centering
\resizebox{\columnwidth}{!}{%

\begin{tabular}{ l|ll|llll }
 \hline
 & \multicolumn{2}{c|}{in-domain} &  \multicolumn{4}{c}{out-of-domain}  \\ 
 & \multicolumn{2}{c|}{SquAD}  & \multicolumn{2}{c}{QASRL} & \multicolumn{2}{c}{ZRE} \\ 
 \hline
  & EM & F1 & EM & F1 & EM & F1  \\
 \hline
 base & 70.43 & 79.76 & & 50.01 & & \textcolor{red}{36.18} \\
 +coverage & 71.07 & 80.15 & & \textcolor{red}{52.24} & & \textcolor{red}{35.25}\\

 
\hline
\end{tabular}
}
\caption{Effect of incorporating coverage on the BiDAF QA model.}

\end{table}

==> how.tex <==
\section{How to Better Understand the Question?}
As mentioned, artifacts in existing datasets drives QA models to learn datasets instead of the task itself.


We examined two different approach in order to improve the understanding of the model from the given question: (1) incorporating a more abstract knowledge about the question into the model, i.e., coverage of the question aspects by the answer, and (2) regenerating a full sentence for answering the question instead of only selecting the answer span.





==> rel.tex <==
\section{Related Work}

==> tasks.tex <==
\section{Tasks}
In this paper, we examined different tasks and datasets.
The examined tasks can be classified into two groups including: question answering and natural language inference.

For question answering, we consider the following tasks: (1) reading comprehension, (2) question-answer driven semantic role labeling (QA-SRL) \cite{D15-1076}, and (3) zero-shot relation extraction (ZRE) \cite{K17-1034}.

For the task of natural language inference, we examine various datasets including:

\paragraph{Reading Comprehension.} In this task a question and a related passage is given and the task is to extract the answer span from the passage.
For the task of reading comprehension, we use the the SQuAD dataset \cite{D16-1264}.
The performance of reading comprehension models is measured by the exact match, i.e., , and F$_1$, i.e., , measures.
%The SQuAD and NewsQA datasets are both created using crowdsourcing.
%SQuAD is created based on Wikipedia articles while NewsQA is created based on CNN news articles.

\paragraph{Question-answer driven semantic role labeling.} 
Semantic Role Labeling (SRL) is the task of finding the semantic arguments of a predicate (e.g.,\ verb) as well as their corresponding roles, e.g., agent, patient, instrument, etc.  
\newcite{D15-1076} propose the task of question-answer driven SRL, in which predicate-argument structures are presented using natural question-answer pairs. For instance, in the sentence ``Alan Turing published Intelligent machinery, a heretical theory'', ``published'' is a predicate with two different arguments, i.e., ``Alan Turing'' and ``Intelligent machinery, a heretical theory''. These predicate-argument structures can be presented by the following two question-answer pairs: (1) ``who published something?''-``Alan Turing'', and (2)``what was published?''-```Intelligent machinery, a heretical theory''.
In QA-SRL, a sentence, from which such question-answer pairs are extracted, and the wh-question question are given and the task is to find the answer span from the sentence.

\paragraph{Zero-shot relation extraction.}
\newcite{K17-1034} propose to model the task of relation extraction as a reading comprehension task in which each relation slot is associated with one or more questions.
For instance, the relation $spouse(x,y)$ can be defined by natural questions like ``who did $x$ married?'' or ``who is $x$'s spouse?''.
\newcite{K17-1034} provide a zero-shot relation extraction dataset with the aforementioned setting, in which the test data contains new relation types that have no labeled training examples.

\paragraph{Natural language inference.} 
Given two sentences, i.e., premise and hypothesis,
the task of natural language inference (NLI) is to specify whether the hypothesis entails, contradicts, or is neutral regarding the given premise.
We use different datasets including RTE-3 \cite{W07-1401}, Stanford NLI corpus (SNLI) \cite{D15-1075}, Multi-Genre NLI (MultiNLI) \cite{N18-1101}, Sentences Involving Compositional Knowldedge (SICK) \cite{sick}, as well as the test set that is created by \newcite{P18-2103}, which we would refer to as SNLI-adv.
The premises of the \newcite{P18-2103} dataset are taken from the SNLI dataset and the hypotheses only differ from the premise by one word.
While this dataset is simpler than SNLI, performance of existing NLI models drop significantly on this dataset.

%\squishlist
%\item Stanford NLI corpus (SNLI) \cite{D15-1075}: this dataset is a large crowdsourced dataset annotated with textual entailment information. The creation of this dataset is based on image captions, i.e., annotators were given a caption of an image and were asked to write an alternative caption that entails, contradicts , or is neutral regarding the original caption.
%\item Multi-Genre NLI (MultiNLI) \cite{N18-1101}: this corpus is also a crowd-sourced dataset, which is modeled on the SNLI dataset. The difference is that it covers a range of genres of spoken and written text.
%\item Sentences Involving Compositional Knowldedge (SICK) \cite{sick}: 
%\squishend



